Armed Conflict and Early Human Capital Accumulation: Evidence from Cameroon's Anglophone Conflict

This paper examines the impact of the Anglophone Conflict in Cameroon on human capital accumulation. Using high-quality individual-level data on test scores and information on conflict-related violent events, a difference-in-differences design is employed to estimate the conflict's causal effects. The results show that an increase in violent events and conflict-related deaths causes a significant decline in test scores in reading and mathematics. The conflict also leads to higher rates of teacher absenteeism and reduced access to electricity in schools. These findings highlight the adverse consequences of conflict-related violence on human capital accumulation, particularly within the Anglophone subsystem. The study emphasizes the disproportionate burden faced by Anglophone pupils due to language-rooted tensions and segregated educational systems.

==> TABLE_1AANGFANC.tex <==
Actions involving Ambazonian rebels &       0.003         &       0.002         &       0.014\sym{*}  &       0.014\sym{*}  \\
                                    &     (0.007)         &     (0.007)         &     (0.008)         &     (0.008)         \\
Actions involving Ambazonian rebels &                     &                     &      -0.034\sym{***}&      -0.035\sym{***}\\
\hspace{2cm}$\times$ Anglophone subsystem&                     &                     &     (0.012)         &     (0.012)         \\
R-sq                                &       0.010         &       0.009         &       0.025         &       0.026         \\
Observations                        &        9022         &        9022         &        9022         &        9022         \\


==> TABLE_1Aa.tex <==
fatalitiesAMBMIL    &      -0.000\sym{**} &       0.000\sym{***}&      -0.000\sym{**} &       0.000\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
R-sq                &       0.078         &       0.553         &       0.064         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_1BANGFANC.tex <==
Actions involving Ambazonian rebels &       0.002         &       0.002         &       0.015\sym{**} &       0.015\sym{**} \\
                                    &     (0.006)         &     (0.006)         &     (0.007)         &     (0.008)         \\
Actions involving Ambazonian rebels &                     &                     &      -0.034\sym{***}&      -0.035\sym{***}\\
\hspace{2cm}$\times$ Anglophone subsystem&                     &                     &     (0.011)         &     (0.011)         \\
R-sq                                &       0.013         &       0.013         &       0.027         &       0.028         \\
Observations                        &        9022         &        9022         &        9022         &        9022         \\


==> TABLE_1Ba.tex <==
fatalitiesAMBMILpc  &      -0.027\sym{***}&       0.006\sym{***}&      -0.023\sym{***}&       0.010\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
R-sq                &       0.080         &       0.553         &       0.065         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_1DS.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)&         (9)\\
\midrule
\emph{\textbf{Education Results (PASEC)}}&            &            &            &            &            &            &            &            &            \\
Reading results&        4585&        54.6&         9.5&        2305&        51.5&         9.0&        2280&        57.8&         9.0\\
Maths results&        4585&        51.5&         8.5&        2305&        48.6&         7.8&        2280&        54.3&         8.2\\
\emph{\textbf{Armed conflict (ACLED)}}&            &            &            &            &            &            &            &            &            \\
Events involving any group&        4593&     20323.9&     18053.2&        2309&     11012.6&     16193.6&        2284&     29737.2&     14632.5\\
Events involving separatists&        4593&      1458.1&      3351.4&        2309&      2891.9&      4267.4&        2284&         8.5&         4.6\\
Events involving the Army&        4593&      4049.9&      8638.9&        2309&      7549.2&     11127.1&        2284&       512.2&       199.9\\
Fatalities involving any group&        4593&     36630.4&     27952.9&        2309&     23767.9&     34934.8&        2284&     49633.8&      1157.3\\
Fatalities involving separatists&        4593&      1376.2&      3230.3&        2309&      2737.5&      4127.1&        2284&         0.0&         0.1\\
Fatalities involving the Army&        4593&     11078.5&     23780.5&        2309&     20760.6&     30602.1&        2284&      1290.4&       244.7\\


==> TABLE_2Aa.tex <==
fatalitiesAMB       &      -0.001\sym{***}&       0.000\sym{***}&      -0.001\sym{***}&       0.000\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
R-sq                &       0.080         &       0.553         &       0.066         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_2Ba.tex <==
fatalitiesAMBpc     &      -0.037\sym{**} &       0.008\sym{***}&      -0.035\sym{*}  &       0.012\sym{***}\\
                    &     (0.002)         &     (0.000)         &     (0.004)         &     (0.000)         \\
R-sq                &       0.129         &       0.553         &       0.129         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_3A.tex <==
fatalitiesMILdt     &      -0.004\sym{***}&      -0.003\sym{***}&      -0.005\sym{***}&      -0.003\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
fatalitiesMIL       &       0.004\sym{***}&       0.003\sym{***}&       0.004\sym{***}&       0.003\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
dT                  &       6.525\sym{***}&       1.175\sym{**} &       5.246\sym{***}&      -0.015         \\
                    &     (0.034)         &     (0.062)         &     (0.031)         &     (0.025)         \\
R-sq                &       0.130         &       0.553         &       0.135         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_3Aa.tex <==
fatalitiesMIL       &      -0.000\sym{**} &       0.000\sym{***}&      -0.000\sym{**} &       0.000\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
R-sq                &       0.078         &       0.553         &       0.063         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_3B.tex <==
fatalitiesMILpcdt   &      -7.858\sym{***}&      -4.781\sym{***}&      -8.266\sym{***}&      -6.048\sym{***}\\
                    &     (0.008)         &     (0.064)         &     (0.008)         &     (0.026)         \\
fatalitiesMILpc     &       7.828\sym{***}&       4.789\sym{***}&       8.240\sym{***}&       6.059\sym{***}\\
                    &     (0.008)         &     (0.064)         &     (0.008)         &     (0.026)         \\
dT                  &       6.442\sym{***}&       1.195\sym{**} &       5.175\sym{***}&       0.016         \\
                    &     (0.034)         &     (0.062)         &     (0.031)         &     (0.025)         \\
R-sq                &       0.130         &       0.553         &       0.135         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_3Ba.tex <==
fatalitiesMILpc     &      -0.030\sym{***}&       0.007\sym{***}&      -0.026\sym{***}&       0.011\sym{***}\\
                    &     (0.000)         &     (0.000)         &     (0.000)         &     (0.000)         \\
R-sq                &       0.080         &       0.553         &       0.065         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_4.tex <==
Fatalities by Ambazonian rebels (rate)&                     &      -1.440         &       1.286         \\
                    &                     &     (3.389)         &     (1.978)         \\
R-sq                &       0.090         &       0.016         &       0.018         \\
Observations        &        1094         &        3343         &        3148         \\


==> TABLE_A1A.tex <==
Events involving Ambazonian rebels&      -0.029\sym{***}&      -8.403\sym{***}&                     &                     \\
                    &     (0.008)         &     (1.718)         &                     &                     \\
Fatalities by Ambazonian rebels&                     &                     &      -0.054\sym{***}&     -12.481\sym{***}\\
                    &                     &                     &     (0.012)         &     (2.499)         \\
R-sq                &       0.553         &       0.553         &       0.553         &       0.553         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\


==> TABLE_A1B.tex <==
Events involving Ambazonian rebels&       0.016\sym{**} &       0.419         &                     &                     \\
                    &     (0.008)         &     (1.650)         &                     &                     \\
Fatalities by Ambazonian rebels&                     &                     &       0.013         &       0.233         \\
                    &                     &                     &     (0.012)         &     (2.400)         \\
R-sq                &       0.562         &       0.562         &       0.562         &       0.562         \\
Observations        &        4585         &        4585         &        4585         &        4585         \\

